ASTRO-H White Paper - Accreting Pulsars, Magnetars, and Related Sources

As the endpoints of massive star evolution, neutron stars are enigmatic celestial objects characterized by extremely dense and exotic nuclear matter, magnetospheres with positrons (antimatter), rapid rotation and ultra-strong magnetic fields. Such an extreme environment has provided an accessible astrophysical laboratory to study physics under conditions unattainable on Earth and to tackle a range of fundamental questions related to: the aftermath of stellar evolution and the powerful explosions of massive stars, the equation of state and physics of some of the most exotic and magnetic stars in the Universe, the workings of the most powerful particle accelerators in our Galaxy and beyond, and the sources of gravitational waves that are yet to be detected. Recent observations revealed a great diversity of neutron stars, including ultra-strongly magnetized pulsars, referred to as "magnetars", and unusual types of accreting X-ray pulsars. In this white paper, we highlight the prospects of the upcoming X-ray mission, ASTRO-H, in studying these highly magnetized neutron stars.

==> 0.0_cover_page.tex <==
\title{
{\large ASTRO-H White Paper}\\
Accreting Pulsars, Magnetars, \& Related Sources}

\author{
S. Kitamoto (Rikkyo University), T. Enoto (RIKEN, NASA/GSFC), \\
S. Safi-Harb (University of Manitoba),  C. Ferrigno (University de Geneve),  \\ 
M. Chernyakova (Dublin Institute for Advanced Studies), \\
K. Pottschmidt (NASA/GSFC), N. Hell (Remeis Observatory, FAU \& LLNL), \\
M. Kuehnel (Remeis Observatory, FAU), T. Yasuda (Saitama University), \\ 
K. Makishima, T. Nakano, M. Sasano (University of Tokyo), \\
M. Ohno (Hiroshima University), S. Sugita (Ehime University), \\
D. Khangulyan, H. Odaka, T. Yuasa, T. Hayashi (ISAS/JAXA),  \\
T. Kohmura, K. Kaneko (Tokyo University of Science), \\
Y. Terada (Saitama University) and H. Krimm (NASA/GSFC)
}

\maketitle

\begin{abstract}
  As the endpoints of massive star evolution, neutron stars are
  enigmatic celestial objects characterized by extremely dense and exotic
  nuclear matter, magnetospheres with positrons
  (antimatter), rapid rotation and ultra-strong magnetic fields.  Such an extreme
  environment has provided an accessible astrophysical laboratory to study
  physics under conditions unattainable on Earth and
  to tackle a range of fundamental questions related to: the aftermath of stellar
  evolution and the powerful explosions of massive stars, the equation
  of state and physics of some of the most exotic and magnetic stars
  in the Universe, the workings of the most powerful particle
  accelerators in our Galaxy and beyond, and the sources of
  gravitational waves that are yet to be detected.  Recent
  observations revealed a great diversity of neutron stars, including
  ultra-strongly magnetized pulsars, referred to as ``magnetars", and
  unusual types of accreting X-ray pulsars.  In this white paper, we
  highlight the prospects of the upcoming X-ray mission, \textsl{ASTRO-H}, in
  studying these highly magnetized neutron stars.
\end{abstract}

\bigskip






